Language-Guided Traffic Simulation via Scene-Level Diffusion

Realistic and controllable traffic simulation is a core capability that is necessary to accelerate autonomous vehicle (AV) development. However, current approaches for controlling learning-based traffic models require significant domain expertise and are difficult for practitioners to use. To remedy this, we present CTG++, a scene-level conditional diffusion model that can be guided by language instructions. Developing this requires tackling two challenges: the need for a realistic and controllable traffic model backbone, and an effective method to interface with a traffic model using language. To address these challenges, we first propose a scene-level diffusion model equipped with a spatio-temporal transformer backbone, which generates realistic and controllable traffic. We then harness a large language model (LLM) to convert a user's query into a loss function, guiding the diffusion model towards query-compliant generation. Through comprehensive evaluation, we demonstrate the effectiveness of our proposed method in generating realistic, query-compliant traffic simulations.

==> body/1_intro_backup.tex <==
\section{Introduction}

\begin{wrapfigure}{R}{0.5\textwidth}
\centering
\includegraphics[width=0.5\textwidth]{images/overview.pdf}
\caption{\textbf{\small{Overview of \method. A user queries in natural language along with predefined APIs and examples are passed into ChatGPT, which generates a differentiable loss in Python. This loss, combined with the initial scene and sampled noise, is utilized by \method to produce query-compliant trajectories.}}}
\label{fig:overview}
\end{wrapfigure}

% simulation testing -> importance of realism, controllability and user friendly interface -> what we want: realistic traffic simulation with text interface
Due to the high expenses and risks associated with conducting large-scale real-world tests~\cite{nummilesneeded}, AV developers depend on comprehensive simulation testing to develop dependable systems~\cite{waymoreport}. 
For simulators to be most effective, they need to provide \textit{realism} and \textit{controllability} in traffic models, as well as a user-friendly interface. \textit{Realistic} traffic ensures that development and testing done in simulation can be applied to real-world, \textit{controllability} allows for the creation of relevant traffic scenarios to examine specific AV behaviors, and a user-friendly interface minimizes the necessity for excessive manual labor and thus scales up AV testing. However, creating realistic~\cite{Suo_2021_CVPR,bits2022} and controllable~\cite{zhong2022guided} traffic models remains an ongoing challenge, and user friendly interfaces have not yet been explored for traffic generation. 
As a text-based interface is usually considered highly user friendly, enables harnessing previously-inaccessible data sources such as collision reports collected by governmental agencies and vehicle insurers, and supports new simulation capabilities such as reconstructing real-world collision scenarios \cite{nhtsa_crash_viewer}, a text interface to generate realistic traffic simulation is thus desirable.

%As text is the most natural way for communication and is the format for many good resources of challenging scenarios creation such as crash reports \cite{nhtsa_crash_viewer}, a model on realistic traffic simulation with a text-interface is thus desirable.


% challenges of text->traffic; 1.how to design the intermediate representation 2.what traffic model to use to support the representation while resulting realistic traffic
Translating text into traffic simulation is highly challenging as the two have different modalities and no large-scale dataset on text to traffic exists. To tackle similar challenges, recent work on LLMs for robot behaviors~\cite{lin2023text2motion, vemprala2023chatgpt} usually design and provide a series of high-level functions to a LLM and asks the LLM to use these functions to control the robot for achieving a user-specified query. In other words, the high-level functions serve as the intermediate representation between text and robot behaviors. Unfortunately, such approach cannot be directly applied to realistic traffic simulation as it is unclear (1) how to preserve the expressiveness of traffic trajectories with only a few functions, and (2) how to use those functions to generate realistic trajectories. Reusing the APIs of a heuristic traffic simulator \cite{sumo18, carla17, svl21} does not fix its inherent limitation of lacking realism as the agents are still either unresponsive to other traffic participants or insufficiently expressive to appear human-like. Existing data-driven approach \cite{Suo_2021_CVPR, bits2022}, which trains generative models of traffic behavior from large driving datasets, does not provide an accessible interface supporting control via high-level functions. 

% our method first part: language to code;  
To overcome these obstacles, we propose to use an intermediate representation - a differentiable loss function (in code format) reflecting user's intention with respect to trajectories  - as a bridge, dividing the translation from user query to traffic simulation into two steps: text to loss function and loss function to traffic simulation. Given the proven abilities of LLMs to generate code from natural language, they can accurately translate a user's intent into a loss function in code.   

% our method second part: loss function to traffic; necessity of flexible model; diffusion model; limitation of single-agent diffusion with example; our method of multi-agent diffusion and a multi-agent transformer architecture
The second step of converting a loss function into loss minimizing, realistic traffic requires a generative traffic model that can generate realistic traffic and possess sufficient flexibility simultaneously. Recently, diffusion models have demonstrated success in conditional generation tasks across various domains like image~\cite{dhariwal2021diffusion}, language~\cite{li2022nlpdiffusion}, and~behavior\cite{janner2022diffuser, ajay2022conditional}. In particular, CTG~\cite{zhong2022guided} applies a diffusion model into traffic generation due to its capability in distribution modeling and test-time adaptability through so-called \emph{guidance}, which essentially uses a differentiable loss function to iteratively perturb the current generation towards desired properties. As we desire a model to possess both realism and provide flexibility, we thus build our model on top of CTG. As traffic scenario involves the interaction of multiple agents, learning a diffusion model for each one independently as in previous work \cite{janner2022diffuser, zhong2022guided} is likely to result in sub-optimal trajectories. For example, for two close consecutive vehicles on the same lane, modeling them independently might result in collision when the vehicle ahead slows down while the vehicle behind does not. To address this challenge, we propose a multi-agent conditional diffusion model which models all the traffic participants simultaneously and thus avoid the sub-optimal interactions. As we need an architecture for the diffusion to models agents jointly, we introduce a multi-agent spatial-temporal transformer architecture that uses alternate temporal and spatial attention modules to capture the interaction of multiple agents over time. By inherently considering multiple agents, our model enables cohesive and flexible generation of all agents in a scene. Overall, we name our proposed language-guided multi-agent conditional diffusion model, \method (see \Cref{fig:overview}).


% evaluation and summary of contributions
We assess \method on the nuScenes dataset \cite{nuscenes}, demonstrating its ability to follow user-specified natural language constraints and generate realistic trajectories. In summary, our contributions are: \textbf{(1)} a language-guided multi-agent conditional diffusion model for generating realistic traffic that adheres to user-defined rules in natural language, and \textbf{(2)} extensive evaluation comparing \method to state-of-the-art baselines, highlighting its superiority in generating high-quality scenarios.


% One potential solution is to leverage the recent advance of large language models (LLMs) which has been shown promising results in translating text data into a different modality like image~\cite{dalle2, imagen} and code\cite{codex}. However, unlike text-only or text-image applications, traffic simulation require an in-depth comprehension of real-world physics, environmental context, and the ability to carry out physical actions. These challenges extend beyond the original scope of language models, as they need to not only interpret the meaning of a given text but also convert the intent into a logical series of physical actions.

% Recently, diffusion models guided by rules specified in signal temporal logic (STL) have been utilized to produce trajectories that are both realistic and controllable \cite{zhong2022guided}. However, this approach is not scalable as it demands users to be proficient in STL and manually create new STL equations for each desired rule.

% Existing driving simulators typically support replaying recorded driving logs or employing heuristic-based controllers to create agent behaviors via an accessible high-level programming API \cite{sumo18, carla17} or scenario editor UI \cite{svl21}. However, such methods lack \textit{realism}, as the agents are either unresponsive to other traffic participants or insufficiently expressive to appear human-like. To tackle these challenges, recent research trains generative models of traffic behavior from large driving datasets \cite{Suo_2021_CVPR, bits2022}. Although the behaviors generated by these models look reasonable, they only reflect the training data distribution and do not offer a mechanism to \emph{control} the resulting traffic flow.


